Some Considerations on Learning to Explore via Meta-Reinforcement Learning

We consider the problem of exploration in meta reinforcement learning. Two new meta reinforcement learning algorithms are suggested: E-MAML and E-$\text{RL}^2$. Results are presented on a novel environment we call `Krazy World' and a set of maze environments. We show E-MAML and E-$\text{RL}^2$ deliver better performance on tasks where exploration is important.

==> discretized_paper/practical_considerations_for_training_emaml.tex <==
% BCS: Still figuring out where I want to put everything. 
The discussion surrounding E-MAML in the previous sections was quite theoretically motivated. In this section, we discuss some tricks to improve the performance of the E-MAML update. 

\textbf{Bias Transformations:}

\textbf{Multiple inner and outer updates:}

\textbf{Whatever else Ge wants to put here:}
